The Power of Log-Sum-Exp: Sequential Density Ratio Matrix Estimation for Speed-Accuracy Optimization

We propose a model for multiclass classification of time series to make a prediction as early and as accurate as possible. The matrix sequential probability ratio test (MSPRT) is known to be asymptotically optimal for this setting, but contains a critical assumption that hinders broad real-world applications; the MSPRT requires the underlying probability density. To address this problem, we propose to solve density ratio matrix estimation (DRME), a novel type of density ratio estimation that consists of estimating matrices of multiple density ratios with constraints and thus is more challenging than the conventional density ratio estimation. We propose a log-sum-exp-type loss function (LSEL) for solving DRME and prove the following: (i) the LSEL provides the true density ratio matrix as the sample size of the training set increases (consistency); (ii) it assigns larger gradients to harder classes (hard class weighting effect); and (iii) it provides discriminative scores even on class-imbalanced datasets (guess-aversion). Our overall architecture for early classification, MSPRT-TANDEM, statistically significantly outperforms baseline models on four datasets including action recognition, especially in the early stage of sequential observations. Our code and datasets are publicly available at: https://github.com/TaikiMiyagawa/MSPRT-TANDEM.

==> _memo_fig_and_table_example.tex <==
\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

==> _todo_deadlines.tex <==
Memo:
20210426 
Move Figure 5 (and Figure 2) to Appendix.


1 Multiclass classification via DRE.
To the best of our knowledge, the present work is the first to attack the multiclass classification problem from density ratio (matrix) estimation (multiclass classification via density ratio estimation) (strictly speaking, early multiclass classification via DRME using multiclass labels). と言いたいが本当だろうか？
(cf. ``Density-ratio estimation via classification is a cornerstone of unsupervised learning. ... It consists of estimating the ratio p/q from their samples without separately estimating the numerator and denominator. [Telescoping Density-Ratio Estimation - NeurIPS]'')

first to attack early \textit{multiclass} classification of time series from density ratio estimation
はほんと。

結論、
Correct: To the best of our knowledge, MSPRT-TANDEM is the first DRE-based model for early multiclass classification.
Correct: Although there are a number of papers about multiclass classification in deep learning community, to the best of our knowledge, MSPRT-TANDEM is the first DRE-based model for multiclass classification in deep learning.
{sugiyama, TIS2010, superfast} proposes multiclass classification via DRE (conditional density estimation) with a \textit{non-DNN-based}, kernel method \footnote{It is controversial to say that {superfast} is a DRE-based model, because if estimating the posterior $p(y|x)$ is regarded as DRE ({DDE paper} says so), all the DNN models trained by minimizing the cross-entropy loss are regarded as performing DRE (because cross-entropy minimization is equivalent to KLD minimization between $p(y|x)$ and $\hat{p}(y|x)$). However, no researchers are aware that they perform DRE at all.}. (Concern: If we say this conditional density estimation is DRE, all the DNNs trained by minimizing cross-entropy loss are DRE models.........uh..........(but MS (in his email and DDE paper\cite{DDE}) really said {superfast} is DRE...))
{Moustakides&Basioti} and {SPRT-TANDEM} perform \textit{binary} classification via DRE (likelihood ratio and local statistic estimation) with neural networks.

Comment: MSPRT-TANDEM is based on the LSEL and MSPRT, both of which have strong theoretical support (consistency, hard class weighting, guess-aversion, and asymptotic optimality).
Besides, our empirical study shows that MSPRT-TANDEM outperforms baseline models, which include conventional, binary DRE models extended to DRME and non-DRE-based models.
（※However, one might not consider that our approach (multiclass classification via density ratio estimation) is a good strategy because DRE is generally more difficult task than multiclass classification. Our work is worth it. Using density ratios, we conduct \textit{early} multiclass classification of time series.）

Conclusion after surveying papers on conditional density estimation and likelihood ratio classifiers:
MSPRT-TANDEM is the first model for likelihood ration estimation-based early multiclass classification in deep learning
(w/o early: likelihood ratio classifier. but are they really with DL?) 
(w/o multiclass: Moustakides, Ebihara) (conventional models: binary classification)
(w/o DL: likely exist e.g. SPRT papers with kernel density estimation?????????)
(LRE->DRE: many DNN-based conditional density estimation papers)
(Conventional models for early classification via DRE (including posterior density estimation, not only likelihood ratio estimation) are non-DNN-based or restricted to binary classification. MSPRT-TANDEM is the first likelihood ratio estimation-based model for early multiclass classification in deep learning).

Title: "Early Multiclass Classification via Sequential Density Ratio Matrix Estimation for Speed-Accuracy Optimization"

DRE via binary classification: [Sugiyama series]\cite{sugiyama2012Density_Ratio_Estimation_in_Machine_Learning}\cite{sugiyama2010density} (called probabilistic classification approach)
DRE via multiclass classification: [Multitask paper]\cite{bickel2008multitask_HIV_DRE_via_multiclass_classification}
binary classification via DRE: [Moustakides&Basioti,2019]\cite{moustakides2019training}[Ebihara+,2021]\cite{SPRT-TANDEM}
multiclass classification via DRE: Ours, [Sugiyama, TIS2010, Superfast]\cite{sugiyama2010superfast_DRE_or_not}

LSIF original \cite{kanamori2009least_LSIF_original}, uLSIF+CNN (with the pairwise sampling) \cite{nam2015direct_uLSIF_for_CNN}
KLIEP orginal \cite{sugiyama2008direct_KLIEP_original}, DSKL and BARR \cite{khan2019deep_DSKL_BARR_original}
NN-RuLSIF \cite{hushchyn2020generalization_NN-RuLSIF}

ECOC org \cite{dietterich1994solving_ECOC_original}

Telescopoing paper \cite{rhodes2020telescoping_DRE} enhance the performance and improve stability but consumes huge memory when the number of class is large, because telescopoing requires multiple DREs for a single class.

2
TANDEM vs TANDEMwO Gaussian regime. Dimension, SNR, ... ?
TANDEMwO is memory-efficient and has no grad conflict.
Presentation order.
We construct our model on top of SPRT-TANDEM => MSPRT-TANDEM.

-V1: Disadvantages of naively extending DRE methods to DRME: Consider a naive extension of uLSIF. It is infeasible to directly optimize the original objective, because DNNs require a huge computational budget to compute the objective function using the whole training set. Therefore, the SGD should be used for efficient training. However, if the number of classes or the imbalance ratio is large, mini-batches are likely to include only a subset of the classes, meaning that the first and/or second terms in the objective are absent in a mini-batch, which leads to instability or slow convergence of the SGD. We may circumvent this problem by using a local minimizer of the objective and \textit{pairs} of examples (as done in \cite{nam2015direct} for binary DRE). However, such a sampling method causes the explosion of the sample size especially when the number of classes is large.
-V2: Introduction of uLSIF: not bounded below. asymmetry of demom and nume, leading to imbalance vulnerability. Our symmetric sum wrt k,l relaxes these problems: now bounded and symmetric. But our LSEL is better than uLSIF!!

- Real-world datasets often suffers from class-imbalance \cite{}. A simple solution to it is to use \textit{loss weighting}, or \textit{cost-sensitive learning} \cite{elkan2001foundations_cost-sensitive_learning}, to enhance the gradient scale of minority examples. Such an extension of the LSEL can be defined as ...
where $C$ is a cost matrix, which enables us to assign an arbitrary cost (weight) to each class, at the expense of the consistency: $\hat{\la}$ does not necessarily converge to $\la$ unless $C$ is proportional to the prior ratios. However, we prove that the cost-sensitive LSEL is \textit{guess-averse} \cite{beijbom2014guess-averse} and therefore can learn discriminative "scores" $\hat{\la}$ from imbalanced datasets. Guess-aversion is defined as follows: ...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To further compare the LSEL with other models, we propose MSPRT-TANDEM, which is build on a modern DNN-based model for early classification, SPRT-TANDEM \cite{SPRT-TANDEM}. We generalize the \textit{TANDEM formula} and \textit{multiplet loss} proposed in \cite{SPRT-TANDEM} to multiclass classification and use them along with the LSEL. The overall architecture, MSPRT-TANDEM, is tested on four datasets with other baseline models and shows better generalization statistically significantly. 
Before proceeding to the experiment section, we modify the TANDEM formula and multiplet loss to multiclass classification and introduce another formula that solves a problem inherent to the TANDEM formula.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

3 Others
- Include all the comments by reviewers.
- how to choose threshold: another option? (SNRとか計算する？)
- comparison of TANDEM approximation with other approximations, e.g., SkipRNN etc.
- beyond a simple iid score average: if random hitting time allowed, SPRT is the best.
- guess-averse loss (LSEL) vs non-guess-averse loss (KLIEP, uLSIF, RuLSIF) on imbalanced dataset.
- D.3の最後のexplains why recently proposed log-sum-exp-type...を本文へ回す
- TANDEM
- multipletの記述を軽くし3.7へ。ablationをappendixへ。
- 3.5 there are the localized class signature (or gradual change) and gradient vanishing problems. We use the following approximation [oblivion formula] (oblivionから名前変えたい). 




% CMT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Thank you for submitting your work to ICML 2021. Please read the following instructions carefully.

Author Registration. Every author of your paper must complete CMTs user information and personal conflict forms by Feb 4 AOE (paper submission deadline). Papers missing this information will be rejected without review.

Changes after abstract submission. You are required to submit a title and abstract by Jan 28 AOE, and the full paper by Feb 4 AOE. Neither the title nor the abstract should be modified by more than 50\% in Levenshtein distance from the version submitted to the system on Jan 28. Submissions that do not satisfy this requirement may be rejected without review. The list of authors cannot be changed after the submission deadline.

Topic area selection. In the submission process, you will be asked to fill in radio buttons selecting topic areas for your paper. Please focus especially on the technical expertise needed to evaluate your paper. Pick topic areas that will help find reviewers who can confidently evaluate your paper.

Questionnaires. During the submission, you also need to answer all questions in the Submission Questions from, and the Reproducibility Questions form.

Supplementary files. You can submit supplementary material until Feb 11 AOE. The purpose of supplementary material is simply to assist reviewers. However, that reviewers are not required to consult supplementary material, so your main PDF should contain everything essential for the evaluation of your paper. Supplementary material must be in the form of a PDF or a ZIP file.

For additional information, please refer to the CFP (https://icml.cc/Conferences/2021/CallForPapers) and ICML 2021 Style & Author Instructions (https://icml.cc/Conferences/2021/StyleAuthorInstructions).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

		* Algorithms		                            	* Deep Learning
		Active Learning		                        	Adversarial Networks
		Adversarial Examples	    	            	Architectures
		Algorithms Evaluation	                		Bayesian Deep Learning
		AutoML		                                	Embedding and Representation learning
		Boosting and Ensemble Methods	        		Generative Models
		Clustering		                            	Optimization for Deep Networks
		Collaborative Filtering	    	            	Others
		Components Analysis (e.g., CCA, ICA, LDA, PCA)	*   Optimization
		Continual Learning		                    	Combinatorial Optimization
		Crowdsourcing		                         	Convex Optimization
		Dimensionality Reduction	            		Derivative Free Optimization
		Kernel Methods		                        	Distributed and Parallel Optimization
		Large Scale Learning	    	            	Non-Convex Optimization
		Metric Learning		                        	Others
		Multimodal Learning		                    	Stochastic Optimization
		Multitask, Transfer, and Meta Learning	    	* Probabilistic Methods
		Networks and Relational Learning		    	Approximate Inference
		Online Learning Algorithms		            	Bayesian Methods
		Optimal Transport		                    	Causal Inference
		Others		                                	Gaussian Processes and Bayesian non-parametrics
		Ranking and Preference Learning		        	Graphical Models
		Semi-Supervised Learning		            	Monte Carlo Methods
		Sparsity and Compressed Sensing		        	Non-parametric models
		Spectral Methods		                    	Others
		Structured Prediction	            	    	Probabilistic Programming
		Supervised Learning		                    	Robust statistics
		Time Series and Sequences	            		* Reinforcement Learning and Planning
		Unsupervised Learning		                	Bandits
		* Applications		                        	Deep RL
		Activity and Event Recognition	                Multi-Agent RL
		Audio and Speech Processing		            	Others
		Computational Biology and Bioinformatics		Planning and Control
		Computational Photography		            	* Social Aspects of Machine Learning
		Computational Social Science		        	AI Safety
		Computer Vision		                        	Fairness, Accountability, and Transparency
		Hardware and Systems		                	Privacy, Anonymity, and Security
		Healthcare		                               	* Theory
		Information Retrieval	            	    	Computational Learning Theory
		Music Modeling and Analysis		            	Deep learning Theory
		Natural Language Processing		            	Game Theory and Computational Economics
		Neuroscience and Cognitive Science		    	Information Theory
		Others		                                   	Models of Learning and Generalization
		Quantitative Finance and Econometrics			Online Learning Theory
		Recommender Systems		                       	RL, Decisions and Control Theory
		Robotics		                            	Statistical Learning Theory
		Speech Recognition
		Sustainability and Environment
		Web Applications










\section{Memo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Done: 1. Figure Architecture, TANDEM, and TANDEMwO
Done: 2. MS loss and hard class weighting 
Done: 3. Section Experiment
Check: 4. Hparams space {supp_Hyperparameters}
5. Missing Figure selection and save
6. Missing Figure detailed values 
7. Statest
8. Summarize Related Work, Supp Related Work
Done: 9. Abstract
10. Conclusion
11. Code Pruning

12. Summarize LLLR-A to E
13. Summarize Cost-sensitive and Guess-averse
14. Code Anonymization for zip
15. Supp Discussion
====================== Jan. 28, 2021 ========================
0. Anonymous Mail Account
1. Github Repository
2. Refine All Logic
====================== Feb. 4, 2021 ========================

% Replot!!!!!!!!!!!!!!!!!!!
### vs. Compared Methods on NMNIST-H (Fix EARLIEST)
MSPRT-TANDEM vs. LSTM-s vs. LSMT-m vs. EARLIEST lam=1e-2 vs EARLIEST lam=1e2 vs NPT
MSPRT-TANDEM = TANDEMwO mult+LSEL

### vs. Compared Methods on NMNIST-100f (Fix EARLIEST)
MSPRT-TANDEM vs. LSTM-s vs. LSMT-m vs. EARLIEST lam=1e-2 vs EARLIEST lam=1e-4 vs NPT
MSPRT-TANDEM = TANDEM mult+LSEL

### Mult vs. LSEL vs. Combo. on NMNIST-H
with M-TANDEMwO

### Table
- App: DetalExperiment; Add the ablation values table.
% Replot!!!!!!!!!!!!!!!!!!!





\section{Figure and Table for ref}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=\columnwidth]{./MSPRT}}
    \caption{
        caption
        } \label{fig: MSPRT}
    \end{center}
    \vskip -0.2in
\end{figure}

\begin{figure}[h]
    \vskip 0.2in
    \begin{minipage}[b]{1.0 \linewidth}
        \centering
        \includegraphics[width=\columnwidth, keepaspectratio]
        {./MSPRT}
    \end{minipage}\\
    \begin{minipage}[b]{1.0 \linewidth}
        \centering
        \includegraphics[width=\columnwidth, keepaspectratio]
        {./MSPRT}
    \end{minipage}
    \caption{a}\label{reg_poly}
    \vskip -0.2in
\end{figure}


%Note use of \abovespace and \belowspace to get reasonable spacing above and below tabular lines.
\begin{table}[t]
\caption{
    Classification accuracies for naive Bayes and flexible Bayes on various data sets.
} \label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
    \toprule
    Data set & Naive & Flexible & Better? \\
    \midrule
    Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
    Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
    Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
    Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
    Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
    Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
    Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
    Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
    \bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


\section{確認事項}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
以下、
Meeting Dates, 
CFPs, 
Style & Author Instructions, 
Submission & Formatting Instructions
の４つ抜粋
=========================================================================
ICML 2021 Meeting Dates (https://icml.cc/Conferences/2021/Dates)
The Thirty-eighth annual conference is held Sun Jul 18th through Sat the 24th, 2021 at Virtual Conference Only.

- Abstract Submission Deadline	
    Jan 28 (Anywhere on Earth) (1/28 23:59)
    = Jan 29 20:59 at Tokyo

- Paper Submission Deadline	
    Feb 04 (Anywhere on Earth) (2/4 23:59)
    = Feb 05 20:59 at Tokyo

(In CMT paper submission form: "Supplementary files. You can submit supplementary material until Feb 11 AOE.")
    Feb 11 (AOE) (2/11 23:59)
    = Feb 12 20:59 at Tokyo

- Author Feedback Opens	
    Mar 18 12:00 AM PDT (3/18 12:00)
    = Mar 19 9:00 at Tokyo

- Author Feedback Closes	
    Mar 23 (Anywhere on Earth) (3/23 23:59)	
    = Mar 24 20:59 at Tokyo

- Author Notification	
    May 08 12:00 AM PDT (5/8 12:00)
    = May 09 9:00 at Tokyo

- Camera Ready	
    Jun 10 (Anywhere on Earth) (6/10 23:59)
    = Jun 11 20:59 at Tokyo 
    
* Anywhere on Earth +21hours = Tokyo

=========================================================================
Call for Papers (https://icml.cc/Conferences/2021/CallForPapers)

- ↓このURLから入るとdomain conflictsの入力画面に飛ぶので入力お願いします。
> Abstracts and papers can be submitted through CMT: https://cmt3.research.microsoft.com/ICML2021/
  

- Neuroscienceへの機械学習の応用という形でneuroも含まれてるんですね。
> Topics of interest include (but are not limited to):
    - General Machine Learning (active learning, clustering, online learning, ranking, reinforcement learning, semi-supervised learning, time series analysis, unsupervised learning, etc.)
    - Deep Learning (architectures, generative models, deep reinforcement learning, etc.)
    - Learning Theory (bandits, game theory, statistical learning theory, etc.)
    - Optimization (convex and non-convex optimization, matrix/tensor methods, sparsity, etc.)
    - Probabilistic Inference (Bayesian methods, graphical models, Monte Carlo methods, etc.)
    - Trustworthy Machine Learning (accountability, causality, fairness, privacy, robustness, etc.)
    - Applications (computational biology, crowdsourcing, healthcare, neuroscience, social good, climate science, etc.)

    
- DecisionされるまでSNSなどでの宣伝禁止。arXivなどのpreprintへの投稿や限られたaudienceへのtalkは可。
> Authors are allowed to post versions of their work on preprint servers such as Arxiv. Also they are allowed to give talks to restricted audiences on the work(s) submitted to ICML during the review.
ICML strongly discourages advertising the preprint on social media or in the press while under submission to ICML. Under no circumstances should your work  be explicitly identified as ICML submission at any time during the review period, i.e. from the time you submit the abstract to the communication of the accept/reject decisions.
    

- 再現性とコードは効く！
> Reproducibility of results and easy availability of code will be taken into account in the decision-making process.

=======================================================================
Style & Author Instructions (https://icml.cc/Conferences/2021/StyleAuthorInstructions)
LaTeX style files is here (https://media.icml.cc/Conferences/ICML2021/Styles/icml2021_style.zip).

- Ref抜きで8ページｗｗｗ Refと謝辞込みで12ページｗｗｗ文字の基本サイズを変えないように。
> Paper Length: Submitted papers can be up to eight pages long, not including references, and up to twelve pages when references and acknowledgments are included. The use of 10-point Times font is mandatory.


- supplementary manuscriptとコードが提出可。
> Authors have the option of submitting one supplementary manuscript containing further details of their work and a separate file containing code that supports experimental findings; it is entirely up to the reviewers to decide whether they wish to consult this additional material.


- コード提出は必須。
> To foster reproducibility, we highly encourage authors to submit code.


- 自分の論文を三人称として引用するのはできるだけやめてくれとのこと。無理やぞ？
> please refer to your prior work in the third person wherever possible, 


- ネット上に著者のIDが推測できそうな情報があってもdouble-blindを破ったとは見做さない。そらそうだ：でなければarXivもだめになる。
> A reviewer may be able to deduce the authors’ identities by using external resources, such as technical reports published on the web. The availability of information on the web that may allow reviewers to infer the authors’ identities does not constitute a breach of the double-blind submission policy.


- Anonymous Githubではなく、anonymous account作ってrepo作ってそこにコード置きましょうか。コードをzipで固めたものをsupplementaryでドンと投げるよりgithubのUIで見やすい形でreviewersに見える方が良いと思うので。README.mdを工夫すると見栄えもよくなるし。「ICML2021のreviewingに関係する操作以外の一切の操作を禁じる」「This repository will be made private upon the author notification」と書けばよいでしょう。
- ただし、submission deadline以降は一切ファイルを更新できないbranchにしなければならないそうです。
- また、supplのzipにはgithub URLだけ書いたtext fileを含めなければならないそうです。
- また、sensitive datasetはsubmitしなくても斟酌してもらえる模様。
> Submission of code through anonymous github repositories is allowed; however, they have to be on a branch that will not be modified after the submission deadline. Please enter the github link in a standalone text file in a submitted zip file. Finally, we understand that many of our authors work with highly sensitive datasets, and are not asking for private data submission. ...
... The supplementary material could be submitted as either a zip file or a pdf.

> supplはpublishされない！のでsupplはどこかよそのweb siteに置いて、final ver.にはそのURLを書くことになる！
- Supplementary material will not be published or archived. If you want to include it in a final version of the paper, you must put it on a web site and reference the site in the final version of your paper.


- 査読者のマッチングはこう決まるんですね。TPMSとOpenReview。
> Reviewer Matching: ICML uses the Toronto Paper Matching System (TPMS) and OpenReview in order to assign submissions to reviewers and area chairs. Both software packages compute similarity scores between ICML submissions and reviewers’ papers. ... (Note that OpenReview is used only for matching; your paper will not be made public.)



- Author feedbackで答えるべきは以下の通り。なので最初に「レビューありがと」「改善点指摘ありがと」「すべてに返事できない」「author instructionに従ってuncertainなとこに絞ってコメントしていくよ」と書くと良さそう。
> There is no need to respond to every minor question or suggestion for improvement. Rather, the response is a good opportunity for addressing issues like a reviewer’s uncertainty about a point, a reviewer making an incorrect assumption, or a reviewer misunderstanding a part of the paper. 


- 一応code of conduct。やべぇreviewrいたらrebuttalで使うかも？
> ICML CoC: https://icml.cc/public/CodeOfConduct


=====================================================================
Submission and Formatting Instructions (example_paper.pdf)
より詳しいフォーマットの情報。
！！！投稿前に再度example_paper.pdf確認の必要あり！！！


- アブストは 4-6 sentences !!
> Abstracts must be a single paragraph, ideally between 4–6 sentences long. Gross violations will trigger corrections at the camera-ready phase.


- ref抜き8ページ。acceptされたら9ページ。(double columns)
> Submitted papers can be up to eight pages long, not
including references, plus unlimited space for references. Accepted papers can be up to nine pages long,
not including references, to allow authors to address
reviewer comments.


- In 10 point Times font. Type-1 fonts
> Your paper should be in 10 point Times font.
> Make sure your PDF file only uses Type-1 fonts.


- は？まじか。fig. captionは下。Tab.captionは上。図のタイトルは図中に載せてはいけない。
> Place figure captions under the figure (and omit titles
from inside the graphic file itself). Place table captions
over the table.


- 複数citeするときは時系列順！！！忘れないようにしないと。
> Place multiple citations in chronological order.


- はい。
> Submissions will not be accepted in
Word format or any format other than PDF. Really. We’re
not joking. Don’t send Word.


- 画像のデータフォーマットは、plot = .pdf, sharp graphics = .png, photo = .jpg
> Graphics files should be a reasonable size, and included
from an appropriate format. Use vector formats (.eps/.pdf)
for plots, lossless bitmap formats (.png) for raster graphics
with sharp lines, and jpeg for photo-like images.


- hyperref (ハイパーリンク)がなんか問題起こすのなら消してもいいよとのこと。
> The style file uses the hyperref package to make clickable links in documents. If this causes problems for you,
add nohyperref as one of the options to the icml2021
usepackage statement.


- \subsubsubsectionは使っちゃダメ。\subsubsectionまで。
> Please use no more than three levels of headings.


- paragraph頭のindentはしない：どうせline breakが入るからいらない。
> Do not indent the first
line of a given paragraph, but insert a blank line between
succeeding ones.


- 脚注はfull sentenceで書く。
> Footnotes should be complete sentences


- 図の線は0.5 point以上の太さで！！暗い色を使わなければならない。
> Lines should be dark
and at least 0.5 points thick for purposes of reproduction,
and text should not appear on a gray background.


- 図中の文字結構小さくて読みにくいｗ
> example_paper.pdf Figure 1. (https://media.icml.cc/Conferences/ICML2021/Styles/example_paper.pdf)


- 図のタイトルはキャプションに書け。
> Do not include a title inside the figure; instead, the caption should serve this function.


- columnの真ん中に図を入れることはできない(?)。上端か下端に。
- columnをぶち抜くデカい図(two-column figure)を入れる時はfigure*環境でcolumnの上端か下端に入れる。
- 表に関しても同様。
> You may float figures to the top or bottom of a column, 
and you may set wide figures across both columns
(use the environment figure* in LATEX). Always place
two-column figures at the top or bottom of the page. ...
... Again, you may float
tables to a column’s top or bottom, and set wide tables
across both columns. Place two-column tables at the top or
bottom of the page.


- Pseudo-codeはalgorithm 環境で。
> If you are using LATEX, please use the “algorithm” and “algorithmic” environments to format pseudocode.


- reference formatはAPA。自動でそうなるはず。
Please use APA reference format regardless of your formatter or word processor. If you rely on the LATEX bibliographic
facility, use natbib.sty and icml2021.bst included
in the style-file package to obtain this format.


- 基本的なciteの仕方！！ et al.は3人以上あるいは既にall authorsをリストし終わっている場合のみ。
> If the authors’ names are included in the
sentence, place only the year in parentheses, for example
when referencing Arthur Samuel’s pioneering work (1959).　
Otherwise place the entire reference in parentheses with the
authors and year separated by a comma (Samuel, 1959).
List multiple references separated by semicolons (Kearns, 1989;
Samuel, 1959; Mitchell, 1980). Use the ‘et al.’ construct
only for citations with three or more authors or after listing
all authors to a publication in an earlier reference (Michalski
et al., 1983).


- 自分の論文は三人称で引用する。
> Authors should cite their own work in the third person in
the initial version of their paper submitted for blind review.


- referenceに必要な情報がちゃんと入っているかexample_paper.pdfの例を確認する。
> The references at the end of
this document give examples for journal articles (Samuel,
1959), conference publications (Langley, 2000), book chapters (Newell & Rosenbloom, 1981), books (Duda et al.,
2000), edited volumes (Michalski et al., 1983), technical
reports (Mitchell, 1980), and dissertations (Kearns, 1989).


- 著者名や論文のタイトルの大文字小文字がよく事故るので確認必須。
> If using bibtex, please protect capital letters of names and abbreviations in titles, for
example, use {B}ayesian or {L}ipschitz in your .bib file


- 文献アルファベット順！これ自動でなるのか？
> Alphabetize references by the surnames of the first authors,
with single author entries preceding multiple author entries.
Order references for the same authors by year of publication,
with the earliest first



=======================================================================================
参考：Reproducibility checklist in CMT

• For all models and algorithms presented, check if you include:
A clear description of the mathematical setting, algorithm, and/or model.
Yes No Not Applicable
A clear explanation of any assumptions.
Yes No Not Applicable
An analysis of the complexity (time, space, sample size) of any algorithm.
Yes No Not Applicable
A link to a downloadable source code, with specification of all dependencies, including external libraries.
Yes No Not Applicable

• For any theoretical claim, check if you include:
A statement of the result.
Yes No Not Applicable
A clear explanation of any assumptions.
Yes No Not Applicable
A complete proof of the claim.
Yes No Not Applicable

• For all datasets used, check if you include:
A complete description of the data collection process, including sample size.
Yes No Not Applicable
A link to a downloadable version of the dataset or simulation environment.
Yes No Not Applicable
The details of train / validation / test splits.
Yes No Not Applicable
An explanation of any data that were excluded, description of any pre-processing step.
Yes No Not Applicable

• For all reported experimental results, check if you include:
The range of hyper-parameters considered, method to select the best hyper-parameter configuration, and specification of all hyper-parameters used to generate results.
Yes No Not Applicable
The exact number of training and evaluation runs.
Yes No Not Applicable
A description of how experiments were run, and any differences from results reported in previous work.
Yes No Not Applicable
A clear definition of the specific measure or statistics used to report results.
Yes No Not Applicable
The average runtime for each result, or estimated energy cost.
Yes No Not Applicable
A description of the computing infrastructure used.
Yes No Not Applicable

＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝＝
！！！！！！！！！！！！！！！！！！！！
！！！！！！！確認事項！！！！！！！！！
！！！！！！！！！！！！！！！！！！！！
0. 全員CMTのユーザー情報とconflict埋めた？
1. Meeting Dates を確認してviolationがないか一つ一つ直接確認。
2. CFPs を確認してviolationがないか一つ一つ直接確認。
3. Style & Author Instructions を確認してviolationがないか一つ一つ直接確認。
4. Submission & Formatting Instructions: example_paper.pdf を確認してviolationがないか一つ一つ直接確認。
5. Paperはanonymizeされている？
6. Codeはanonymizeされている？
7. Codeのライセンスは大丈夫？
8. zipにしたsupplは解凍できる？
9. Paper古いバージョンを投稿してない？
10. Suppl古いバージョンを投稿してない？
11. Acknowledgementは含まれていない？
12. Place multiple citations in chronological order.










\section{伊藤さんのコメ}
%  ICLR2021への採録，おめでとうございます！　論文を読みましたが，
%  大作ですね．
%  読んでみてわかりにくかったところがありました．以下となります．
%  - Eq. (2) において，\lambda_{\tau^\ast} が -a_0 から a_1 の
%  ときは，どうなるのでしょうか？ Fig. 1 の undecided の状態だと
%  思いますが， decision rule d^\ast には含まれないのでしょうか？
%  decided ではないので含まれないとは思いますが，気になりました．
%  - Eq. (2) で sequential data X^{(1,T)} が出てきますが，3 節の
%  The TANDEM formula まで説明が出てきませんでした． Eq. (2) で
%  X の説明を入れた方がわかりやすいです．
%  - Fig. 2 ですが，ブロック図は 1 次で描かれていますが，上の数式
%  は N 次なので，少し混乱しました．
%  - すごく細かいことですが，5ページの Density fitting のところで
%  杉山先生の文献の引用が他とスタイルが異なります．括弧です．
%  教えてもらいたいんですが，early classification とは，時間的に
%  早いという意味でしょうか？　（早いより簡単とか単純でしょうか？）
%  具体的に何を求める実験を行ったのでしょうか？　SiWがわかりやすい
%  と思うので例とすると，real と fake の2値分類問題を解かせたで
%  あってますか？　そのときに，何フレームを使って分類精度がどれ
%  くらいかが Fig. 3 のプロットになるでしょうか．その場合，1フレーム目
%  と2フレーム目の間にプロットがありますが，これはなぜでしょうか？
%  Eq. (5) が全体の損失関数ですが，LLR のみと multiplet のみの場合は
%  それくらいの性能になるのでしょうか？　（付録に記載がありましたら
%  申し訳ございません．）
%  時間を考慮した損失関数の提案ということで，面白いなと思いながら
%  読ませていただきました．例えばですが，3D CNN を (2+1)D CNN
%  に分解したときの損失関数として使えたりしないですかね？
%  提案手法の有効性の1つである early decision ではなくなるので，
%  微妙かもしれませんが・・・．
%  マルチタスクへ拡張した場合は，タスクによって速度が異なると
%  思うので，そこのバランスが難しそうですね．単純には，ハイパー
%  パラメータを導入してバランスさせるんですかね．
%  すでにご存じだと思いますが，SiW が公開停止になったようです．
%  データにまずいものが含まれていたみたいですね．新しいバージョン
%  をそのうち公開するから，それを使うようにという連絡がありました．
%  まとまりのない文章になりましたが，参考になれば幸いです．
%  よろしくお願いします．
 
%  ２，３，４番目はその通りだな．修正しましょう．
% なんで気づかなかったし
% あてくしの返信↓
% > 東北大学　伊藤先生
%  >
%  > NECの海老原です．
%  > お忙しい中論文を読んでコメントを書いていただき，どうもありがとうございます！
%  > ちょうどCamera-Ready前なので，本当に助かります．ご意見をもとに修正を加えようと思います．
%  >
%  > 以下，ご質問にお答えします．
%  >
%  >
%  >> - Eq. (2) において，\lambda_{\tau^\ast} が -a_0 から a_1 の
%  >> ときは，どうなるのでしょうか？ Fig. 1 の undecided の状態だと
%  >> 思いますが， decision rule d^\ast には含まれないのでしょうか？
%  >> decided ではないので含まれないとは思いますが，気になりました．
%  >
%  > SPRTは系列データの要素を１つ１つ取得していき，逐次的に対数尤度比λをアップデートします．
%  > 対数尤度比λが2本の閾値-a_0とa_1の間にあるときは，ご指摘のようにundecided状態になります．
%  > このときは，つぎのサンプルを取得し，λをアップデートします．この作業を，閾値に到達するまで繰り返します．
%  > なので，そうですね，Eq.(2)はSPRTの先行研究に倣った表記になっているのですが，
%  > 「クラス１に分類」「クラス０に分類」「分類しない」の3択をdecision ruleにしてもいいと思います．
%  >
%  > なお，実応用上はサンプルサイズは有限であることが多いので，規定のサンプル数に達したらa_1 = a_0 = 0とし,
%  > 強制的に2値分類を行うようにしています．(p.7 l.15あたりに書かれています）
%  >
%  >
%  >> - Eq. (2) で sequential data X^{(1,T)} が出てきますが，3 節の
%  >> The TANDEM formula まで説明が出てきませんでした． Eq. (2) で
%  >> X の説明を入れた方がわかりやすいです．
%  >
%  > 仰る通りです．どうもありがとうございます，最終稿で修正を加えたいと思います．
%  >
%  >
%  >> - Fig. 2 ですが，ブロック図は 1 次で描かれていますが，上の数式
%  >> は N 次なので，少し混乱しました．
%  >
%  > 確かに，数式と齟齬がありますね．こちらも最終稿で修正したいと思います．ありがとうございます．
%  >
%  >
%  >> - すごく細かいことですが，5ページの Density fitting のところで
%  >> 杉山先生の文献の引用が他とスタイルが異なります．括弧です．
%  >
%  > 本当ですね．．．すみません，気づきませんでした．修正を加えます，ありがとうございます．
%  >
%  >> 教えてもらいたいんですが，early classification とは，時間的に
%  >> 早いという意味でしょうか？　（早いより簡単とか単純でしょうか？）
%  >
%  > はい，early-classificationとは，目標精度据え置きでできるだけ少ないサンプル数で分類を行うという意味です．ですので，多くの場合時間的に早いと言っても差し支えありません．
%  > 使用サンプル数を抑えられるので，サンプリングコストの高い系列データ分類問題に適しています．
%  > たとえば医療における診断回数や，軍事・防衛の際の観測回数．我々の場合はゲートレス顔認証システムを被検者が通り抜けるまでに判断を下したいというモチベーションがあります．
%  > SPRTはこのようなearly-classificationの1種として考えることができます．
%  >
%  > ちょっと歴史の話をしますと，SPRTとは元々は第二次世界大戦中にAbraham Waldが開発したもので，精度を保証しつつできるだけ少ないサンプル数で判断ができるという理論保証がある技術でした．
%  > 当時は戦争から返ってきた戦闘機などの兵器を，できるだけ少ない点検で修理するかどうか決定するために使われたようです（戦争はサイエンスを発展させたりするので皮肉なものです）．
%  >
%  > ただし，WaldのSPRTは２つの厳しい仮定を置いていました．１つはサンプルが独立同分布(i.i.d.)に従うこと．もう１つは対数尤度比が既知であることです．
%  > 我々のSPRT-TANDEMでは，ニューラルネットを用いてこれらの条件を緩和し，推定された尤度比を用いてSPRTを行っています．
%  >
%  > 2015年には，サル側頭葉のニューロンの活動が，サルが分類タスクを行うときにSPRTの尤度比のような動きをすることが報告されました．
%  > 私は元々神経科学でPh.D.を取得しており，このあたりの歴史を少し知っていたので，今回deep neural networkの力を借りて実応用しやすいSPRTを開発した，という経緯です．
%  >
%  > なお，通常のearly-classificationでは，「精度を良くするloss」と，「速度を良くするloss」を別々に設定していることが多いですが，
%  > 前述のWaldが尤度比を正確に求めれば精度・速度両方を最適化できると理論で示しているので，我々は尤度比推定lossしか使っていません．
%  > タイトルにある"Simultaneous Optimization"とはこのことを指しています．
%  > すみません，長くなりました．
%  >
%  >
%  >> 具体的に何を求める実験を行ったのでしょうか？　SiWがわかりやすい
%  > と思うので例とすると，real と fake の2値分類問題を解かせたで
%  > あってますか？　
%  >
%  > はい，対数尤度比の逐次推定を行い，その値を元に2値分類問題を解いています．
%  > ちなみにNクラス分類用のアルゴリズムも開発が終了しているので，こちらも将来論文化したいと思っています．
%  >
%  >
%  >> そのときに，何フレームを使って分類精度がどれくらいかが Fig. 3 のプロットになるでしょうか．
%  >
%  > はい，その通りです．
%  >
%  >
%  >> その場合，1フレーム目と2フレーム目の間にプロットがありますが，これはなぜでしょうか？
%  >
%  > 横軸は「平均」フレーム数をプロットしているので，アルゴリズムによっては非整数の値を取りえます．初期値を変えた学習を何回も行い平均値を出しています．
%  > 比較したBaseline手法の１つ，EARLIESTの平均値が1フレーム目と2フレーム目の間にあるので，この位置にプロットがあります．
%  >
%  > 一方，SPRT-TANDEMやLSTM-ｍ，LSTM-ｓといった手法は，閾値の位置によって（ある程度）自由に平均フレーム数を変えられます（その代わり，当然ですが平均フレーム数を固定すれば精度も固定されます）．
%  > ですので，これらの手法に関しては，横軸が整数値になる場所と，EARLIESTの平均フレーム数（小数）に合わせた位置で精度を計算してプロットをしています．
%  >
%  >
%  >> Eq. (5) が全体の損失関数ですが，LLR のみと multiplet のみの場合は
%  >> それくらいの性能になるのでしょうか？　
%  >
%  > Fig.3-eに，片方ずつの場合と両方使った場合のablation test結果が載せてあります．
%  > 傾向として，cross-entropyのみだと小サンプル時の精度がよく，LLLRのみだとサンプルサイズを増やしたときに精度が良くなるようです．
%  >
%  >
%  >> 時間を考慮した損失関数の提案ということで，面白いなと思いながら
%  >> 読ませていただきました．例えばですが，3D CNN を (2+1)D CNN
%  >> に分解したときの損失関数として使えたりしないですかね？
%  >
%  > ちょっと理解していないかもしれませんが，我々の手法は結局尤度比推定lossを提案し，速度はその帰結として保証される，というものなので，
%  > (2+1)D CNNの分解specificに効く損失関数かはわかりません．CNNの出力から尤度比を構成する場合には役立つと思います．
%  >
%  > (2+1)D CNNといえば，APSIPA2020に論文出されてましたね．おめでとうございます！
% >
%  >
%  >> マルチタスクへ拡張した場合は，タスクによって速度が異なると
%  >> 思うので，そこのバランスが難しそうですね．単純には，ハイパー
%  >> パラメータを導入してバランスさせるんですかね．
%  >
%  > マルチタスク拡張，面白そうですね．
%  > 「平均decision速度を学習なしに変更できる（閾値をずらすだけなので）」のはSPRT-TANDEMの１つの強みなので，
%  > 例えばすべてのタスクを同時に終わらせたい，とかであればハイパラなしでもいけるかもしれません．
%  > つまり，閾値の値を変えれば平均終了時間（Fig.3a-cの横軸）を自在に変えられるので，
%  > 遅いタスクは小さい閾値，速いタスクは大きい閾値に設定すれば，ほぼ同時に終わるような状況を作ることは可能だと思います．
%  > ただ，もちろんその場合精度がばらつく可能性が大きいですが．
%  >
%  >
%  >> すでにご存じだと思いますが，SiW が公開停止になったようです．
%  >> データにまずいものが含まれていたみたいですね．新しいバージョン
%  >> をそのうち公開するから，それを使うようにという連絡がありました．
%  >
%  > ！？知らなかったです．．．SiW-MでなくてSiWですか？
%  > ありがとうございます，気をつけます．
%  >
%  >
%  >
%  >> まとまりのない文章になりましたが，参考になれば幸いです．
%  >
%  > 大変有意義な議論をさせていただきどうもありがとうございました！
%  >
%  > 海老原　章記
% ↓伊藤先生の返信（めっちゃ早い）
% 12:58
% NEC 海老原様
%  東北大学の伊藤です．
%  お世話になっております．
%  丁寧な回答，ありがとうございました．疑問点などを含めて理解できました．
%  > たとえば医療における診断回数や，軍事・防衛の際の観測回数．我々
%  の場合は
%  > ゲートレス顔認証システムを被検者が通り抜けるまでに判断を下した
%  いという
%  > モチベーションがあります．
%  > SPRTはこのようなearly-classificationの1種として考えることができ
%  ます．
%  early classification ですが，動画像のように似たようなシーン系列の
%  データに
%  対する早期段階での認識・・・でしょうか．
%  > 私は元々神経科学でPh.D.を取得しており，このあたりの歴史を少し
%  知っていた
%  > ので，今回deep neural networkの力を借りて実応用しやすいSPRTを開
%  発した，
%  > という経緯です．
%  こういうのは，本当に強みだと思います．知っているか知っていないかが
%  大きい
%  ですよね．ぜひぜひ神経科学で得た知識を活用して下さい．
%  3D CNN のところの話は，すみません，メールを送った後にちょっと違うな
%  って思ってました．先ほど書いたような「似たようなシーン系列のデータ」で
%  はなく，ボリュームデータみたいなものに適用できないかなと考えました．
%  スライス画像を動画像で言うフレームとして扱うということです．今回の手法
%  は，分類精度を下げずに早い段階で結果を出すことがポイントなので，そ
%  ういう
%  使い方は難しいな・・・ということで，少しずれた質問をしてしまったという
%  ことでした．
%  APSIPAの論文は大したことがないので，もう少し頑張った手法を考えないと
%  いけないと思ってます．ベースラインとして，(2+1)D CNN ではなく，
%  TSM に置き換えることを考えています．TSM の方がよいらしいです．
%  TSM: Temporal Shift Module
%  https://openaccess.thecvf.com/content_ICCV_2019/papers/Lin_TSM_Temporal_Shift_Module_for_Efficient_Video_Understanding_ICCV_2019_paper.pdf
% あとは，デプスのような特徴量の追加です．なりすまし攻撃の検知に限った
%  話ではありますが，なりすまし画像から推定されるデプスマップがフレーム
%  間でばらつきます．当たり前なんですが，無理矢理デプス推定をしている
%  弊害になります．本物であればばらつきが小さいので，それをうまく利用
%  したいと考えています．
%  マルチタスクへの適用についてですが，Nクラス分類を間違ってマルチタスク
%  と読んでしまいました．ただ，時間をかけてもいいタスクとそうでないタスク
%  があると思うので，うまく重み付けするにはよさそうな気はします．
%  > ！？知らなかったです．．．SiW-MでなくてSiWですか？
%  すみません，SiW-Mでした．SiW Management Team からの連絡だったので，
%  SiWと読んでしまいました・・・申し訳ないです．学生にSiWが使えないって
%  言ってしまったので，訂正しておきます．ありがとうございました．
%  海老原さんに負けないように私たちも一層頑張ろうと思います．
%  よろしくお願いいたします．
% あてくし2投目↓
% 東北大学　伊藤先生
% お世話になっております，NECの海老原です．
% お返事どうもありがとうございました．追加のコメントを加えます．
% >early classification ですが，動画像のように似たようなシーン系列の データに
%  >対する早期段階での認識・・・でしょうか．
% 仰る通りです．ただ，必ずしも"似たような"系列でなくても構いません（必然的に似ることが多いですが）
% 提案手法SPRT-TANDEMに限っては動画像でもいいですし，音声のような連続データから
% sliding windowを使って部分的に取ってきたデータでも構いません（今回の論文中の評価は全て動画ですが）．
% または，１枚の写真のsubregionを逐次的にクロップしてくることで系列データにするなど，多種多様な使い方ができます．
% >こういうのは，本当に強みだと思います．知っているか知っていないかが
%  >大きいですよね．ぜひぜひ神経科学で得た知識を活用して下さい．
% ありがとうございます．神経科学の知見は定性的なものが多くなかなか役に立つものが少ないのですが，
% 側頭葉ニューロンの活動はSPRTでモデル化されていたので応用することができました．
% >3D CNN のところの話は，すみません，メールを送った後にちょっと違うな
%  >って思ってました．先ほど書いたような「似たようなシーン系列のデータ」で
%  >はなく，ボリュームデータみたいなものに適用できないかなと考えました．
%  >スライス画像を動画像で言うフレームとして扱うということです．
% ボリュームデータ．．．なるほど，例えばMRI画像のようなものですよね．
% なるべく少ないスライス数で判断したいという要請があるかどうかだと思います．
% 既にボリュームデータ全てが手元にあるような状況ですと，敢えてその中の数枚だけで
% decisionするモチベーションはあまりないかもしれませんね．全部CNNに突っ込めばいいので．．．
% 1スライスあたりのサンプリングコストが大きい場合だと適用する意義があるかもしれませんね．
% ただ，我々の実験で，３DCNNと同じ枚数を使った場合のSPRT-TANDEMのほうが精度がよくなった，
% というケースもあったので，earliness度外視で単純に精度が向上する場合もあるようです．
% その場合は枚数に関係なく適応する意義があると思います．
% また，話がすこし飛びますが，先述した「1枚の写真のsubregionを逐次的にクロップ」の場合は，
% 写真全体ではなく敢えてlocalな情報だけCNNに見せたいような場合に飛び道具的に使っています．
% このように，色んな使い方ができる手法だと思います．
% >なりすまし画像から推定されるデプスマップがフレーム
%  >間でばらつきます．当たり前なんですが，無理矢理デプス推定をしている
%  >弊害になります．本物であればばらつきが小さいので，それをうまく利用
%  >したいと考えています．
% なるほど，RGB1枚からのデプス推定ということですよね．
% 貴重な知見，ありがとうございます．うちのなりすまし検知チームも，
% また可視光1枚からのなりすまし検知をやるらしいので（今井くん担当かな．．．），
% 留意しておきたいと思います．
